Threshold Queries in Theory and in the Wild

Threshold queries are an important class of queries that only require computing or counting answers up to a specified threshold value. To the best of our knowledge, threshold queries have been largely disregarded in the research literature, which is surprising considering how common they are in practice. In this paper, we present a deep theoretical analysis of threshold query evaluation and show that thresholds can be used to significantly improve the asymptotic bounds of state-of-the-art query evaluation algorithms. We also empirically show that threshold queries are significant in practice. In surprising contrast to conventional wisdom, we found important scenarios in real-world data sets in which users are interested in computing the results of queries up to a certain threshold, independent of a ranking function that orders the query results by importance.

==> 06-related-work-long.tex <==
\section{Related Work}
\label{sec:related-work}

\paragraph{Counting Answers}

A celebrated result by Grohe \cite{Grohe-jacm07} states that, assuming $\mathsf{FPT} \neq \mathsf{W}[1]$, Boolean evaluation is tractable for a class of conjunctive queries iff the cores of the CQs in this class have bounded tree-width. 
%The earliest results relevant to counting query answers were obtained in the context of the homomorphism problem. For a class $\cC$ of relational structures, the problem $\textsf{HOM}(\cC,-)$ is to decide if there is a homomorphism from a given relational structure $\mathbb{A}\in\cC$ into a given arbitrary relational structure $\mathbb{B}$. A celebrated result by Grohe \cite{Grohe-jacm07} states that, assuming $\mathsf{FPT} \neq \mathsf{W}[1]$, $\textsf{HOM}(\cC,-)$ is tractable iff the cores of the structures in $\cC$ have bounded tree-width. 
%
% A precursor of this result is the characterization for \emph{structural} classes $\cC$, that says $\textsf{HOM}(\cC,-)$ is tractable if and only if structures in $\cC$ have bounded treewidth. 
%
%This characterization was lifted to the counting setting by Dalmau and Jonsson \cite{DalmauJ-tcs04}, who proved that, even under weaker complexity-theoretic assumptions, the associated homomorphism counting problem $\#$\textsf{HOM}$(\cC,-)$ is solvable in polynomial time if and only if the structures in $\cC$ have bounded tree-width. 
%
This characterization was lifted to the counting setting by Dalmau and Jonsson \cite{DalmauJ-tcs04}, who proved that, even under weaker complexity-theoretic assumptions, counting answers is tractable for a class of \emph{full} CQs iff the CQs in this class have bounded tree-width;
the easier, positive part was shown earlier by Flum and Grohe \cite{FlumG04}.
% who also investigate fixed-parameter tractability of homomorphism counting. Note that $\mathsf{P}$ under fixed tree-width does not imply $\mathsf{FPT}$ with tree-width as the parameter or even with the size as the parameter, and indeed the obtained results are negative. 
%
%While counting homomorphisms can be seen as counting answers to full CQs (that is, projection-free CQs), 
%A systematic study of the complexity of counting query answers was initiated 
Much more recently, Pichler and Skritek \cite{Pichler_Skritek_2013} showed that in the presence of existentially quantified variables the problem is \sharpP-hard even for acyclic CQs. 
%
% More precisely,  \cite{Pichler_Skritek_2013} shows that counting perfect matchings reduces to counting answers to acyclic CQs via a (strong) subtractive reduction \cite{DurandHK05} with two calls to the oracle. Counting perfect matchings is known to be complete for \sharpP with respect to polynomial-time Turing reductions with a single call to the oracle \cite{Zanko91}. Note that even this is not the same as Karp reductions, because the returned number is further processed before returning. 
This implies that the problem is intractable unless $\mathsf{P}=\mathsf{NP}$. Note that this is in stark contrast with Boolean evaluation, which is tractable not only for acyclic CQs \cite{Yannakakis81}, but also for CQs of bounded tree-width \cite{chekuri2000conjunctive}. 
%
A full characterization of classes of CQs with tractable answer counting is yet missing, but there is a characterization for \emph{structural} classes, where membership depends only on the hypergraph underlying the query; for example, for CQs over directed graphs, if some query belongs to such a class, then each query obtained by reversing directions of some edges must also belong to the class. Durand and Mengel \cite{DurandM15} show that, assuming $\mathsf{FPT} \neq \mathsf{W}[1]$, answer counting can be done in $\mathsf{P}$ for a structural class of CQs iff the queries in the class have bounded tree-width and bounded star-size.
% The latter measures how  quantified variables are connected to free variables. 
%
Thus, counting answers to CQs is  harder than just checking if an answer exists and tractability requires additional assumptions; namely, bounded star-size. However, when the counting problem is relaxed to approximate counting, tractability comes easier. In a very recent paper \cite{arenas2020approximate}, Arenas et al.~show that, assuming $\mathsf{FPT} \neq \mathsf{W}[1]$ and $\mathsf{BPP} = \mathsf{P}$, a structural class of queries admits a fully polynomial-time randomized approximation scheme for counting answers iff the queries in the class have bounded tree-width; that is, the characterization is just like for Boolean evaluation. In this work, we consider a very different relaxation --- counting exactly, but only up to a given threshold --- and we show tractability under the same assumption. 
%Just like in the above work, our notion of tractability is relaxed slightly: measure complexity with respect to the actual value of the threshold, not the length of its binary representation. 
% As long as threshold values are significantly smaller than the size of the database instance, our results provide concrete complexity improvements, even for queries of low arity.

%the query in Proposition~\ref{prop:at-most-hard} has large star-size. These results are after a precise number, not a threshold, and they cover fewer queries that we can hope for. 

%We recall some basic notions. The class \sharpP is the class of function problems closely associated with the \NP class: a function problem $f$ is in \sharpP if there exists a non-deterministic polynomial-time Turing machine $M$ such that $f(x)$ is the number of accepting runs of $M$ on an input $x$. An alternative definition of \sharpP counts the number of witnesses of an input of a \NP problem, and as such it is generalized to other complexity classes. Essentially, for a complexity class $\mathcal{C}$ the class $\mathsf{\#}\mathcal{C}$ consists of counting witnesses to a problem that can be solved with a Turing machine that for a given input guesses (nondeterministically) a witness, which is verified with a $\mathcal{C}$ oracle. For instance, it is known that the combined-complexity of counting answers to projection free conjunctive queries (no existential variables) is \sharpP-complete \filip{citation?}. On the other hand, counting answers to arbitrary conjunctive queries is \sharpNP-complete (query-complexity). \filip{citation?}

%The relationship between \sharpP and \NP can at times be counter-intuitive and below we outline some facts:
%\begin{itemize}
%    \item Counting is very powerful, powerful enough to capture the whole polynomial hierarchy when used as an oracle. It is known that $\P^\sharpP$ contains the whole polynomial hierarchy (Toda's theorem). 
%    \item \sharpP is contained in \PSPACE: by reusing the space, one can enumerate all executions and use a dedicated polynomially-sized counter. 
%    \item In general, a counting problem is as hard as the corresponding \NP decision problem: to solve an \NP decision problem it is enough to know if there is at least one successful execution. More precisely, if a decision problem is \NP-complete, then the corresponding counting problem is \sharpP-complete. 
%    \item The converse does not necessarily hold. For instance 2SAT is in \P yet its counting variant, finding the number of valuations satisfying a 2CNF formula, is \sharpP-complete.
%    \item It is unlikely that \sharpP-complete is tractable. If a \sharpP-complete problem can be solved in polynomial time, then $\P=\NP$. Furthermore, for any \sharpP-complete problem $f(x)$, the decision problem $\{(x,k)\mid f(x) < k\}$ is  \NP-hard under polynomial-time Turing reductions (bisection method), provided that $k$ is given in binary. If $k$ is given in unary, this is no longer the case. For instance, $\{ (x, k) \mid \#\textrm{2SAT}(x) < k\}$ is in \P \cite{Dubois91}. The algorithm constructs a tree of `extendable' partial valuations, level by level, and rejects only when the tree gets more then $k$ branches. The at-least variant and the exact variant can be solved similarly.  Interestingly, the problem UNIQUE SAT, which asks if a given CNF formula has a unique satisfying valuation is known to be \coNP-hard, but is not known to be \NP-hard \cite{BlassG82, Juban99}. It is unlikely that polynomial-time Turing reductions can be replaced with Karp reductions, because the notion of \sharpP-hardness is defined in terms of polynomial-time Turing reductions. In particular, \cite{Pichler_Skritek_2013} shows that counting perfect matchings reduces to counting answers to acyclic CQs via a (strong) subtractive reduction \cite{DurandHK05} with two calls to the oracle. Counting perfect matchings is known to be complete for \sharpP with respect to polynomial-time Turing reductions with a single call to the oracle \cite{Zanko91}, but even this is not the same as Karp, because the returned number is further processed before returning. 
%\end{itemize}


%\cite{Pichler_Skritek_2011} reduces the problem of validating a tgd to counting query answers: $\varphi(\bar{x})\rightarrow\exists \bar{y}.\ \psi(\bar{x},\bar{y})$ is satisfied by an instance iff the two queries $Q_1(\bar{x})=\varphi(\bar{x})$ and $Q_2(\bar{x})=\exists \bar{y}. \varphi(\bar{x})\land\psi(\bar{x},\bar{y})$ return the same number of answers. In the same paper, Pichler and Skritek show that the combined- and query-complexity of tgd validation are both $\Pi^\P_2$-complete. The both complexities become coNP-complete if the tree-width of the body and the tree-width of the head are bounded (independently). Furthermore, if the tree-width of the combined body and head formula is bounded, then query-complexity becomes polynomial (and uses the above reduction to counting query answers). Whether such a constraint has an impact on combined-complexity remains an open question; \cite{Pichler_Skritek_2013} show  that the combined complexity of counting answers to acyclic conjunctive queries with existential variables is \sharpP-complete, which precludes the above reduction from being useful in establishing tractability of the combined-complexity of tgd validation. 

%Because TGDs are a special case of at-least constraints, the negative results carry over. As for positive results it is unclear if a reduction similar to the one above can be proposed for counting constraints. In fact, it seems rather unlikely. While the case of bounded tree-width of the combined head-and-body query can inspire some hope for a subclass of counting constraints with tractable combined-complexity of validation \filip{We can be much more precise than this.}, the practical usefulness of such a subclass is questionable. 

% Related to our work is \cite{ChenD12}, where a classification of quantified CQs is given according to the complexity of the evaluation problem. A much earlier paper on the same topic actually shows that tree-shaped queries with $\forall \exists$ quantifier prefix are \coNP-complete \cite[Theorem 3.4]{GottlobGS05}, which implies our Proposition~\ref{prop:at-least-hard}, and answers the open problem associated with \cite[Theorem 3.6]{Pichler_Skritek_2011} about the combined complexity of TGDs with combined bounded tree-width. 


\paragraph{Enumerating Answers}

Enumeration of answers to CQs was first studied by Bagan, Durand, and Grandjean  \cite{BaganDG07}, who showed that for acyclic CQs one can enumerate answers with linear delay between consecutive tuples. They also introduce the notion of free-connex tree-width of queries, which is a refinement of tree-width that imposes additional strict conditions on the location of free variables in the query, and show that for queries with bounded free-connex tree-width one can enumerate answers with constant delay after polynomial-time preprocessing. This is complemented by a conditional lower bound for self-join-free acyclic CQs: assuming that Boolean $n\times n$ matrix multiplication cannot be realized in time $O(n^2)$, self-join-free acyclic CQs that are not free-connex cannot be enumerated with constant delay and linear preprocessing.
%
The positive result on constant-delay enumeration has been strengthened by replacing tree-width with fractional hypertree-width \cite{OlteanuZ15,DeepK18,KaraO18} and submodular width \cite{BerkholzS19} but always in the free-connex variant. For submodular width there is a conditional lower-bound for self-join-free full CQs, under the exponential time hypothesis (ETH) \cite{Marx13}.
%
Very recent work by Tziavelis et al.~\cite{TziavelisAGRY-pvldb20,tziavelis2020TODS} partially lifts these results to the setting of \emph{ranked enumeration}, where query answers must be enumerated according to a predefined order; the lifted results allow enumeration with \emph{logarithmic} delay and handle  \emph{full} CQs of bounded submodular width as well as free-connex acyclic CQs.
%
%A recent paper \cite{BerkholzS19} pushes it to free-connex bounded submodular width (with FPT preprocessing), and explains well the main results in the field. %\cite{Durand20,BerkholzGS20} would probably be useful, but ACM protects their publications fiercely. 
%
The above results show that also enumeration of answers is harder than testing if an answer exists and --- just like in the case of counting answers --- tractability requires additional assumptions, this time materializing in the use of the free-connex variant of width measures. In this work, we show that knowing beforehand how many answers will be needed makes this additional assumption unnecessary, which again leads to concrete complexity improvements. 

%Enumeration with constant delay can be used to see if a threshold is exceeded or not, but these results are for free-connex variants of the width, so the also cover less that we can hope for. \cite{BaganDG07} also shows that for acyclic queries one can enumerate with linear delay. They do not have a result about bounded tree-width, probably because this would involve polynomial delay, and this did not seem worthwhile. I would bet one could do this, but for us it is probably better to just do counting answers up to a threshold in quasipolynomial time.


%\paragraph{Any$-k$ enumeration} 
% Any$-k$ enumeration is a recent framework allowing to enumerate ranked results of full conjunctive queries (without projection) \cite{TziavelisAGRY-pvldb20}. The idea is to design algorithms that have optimal guarantees (in terms of the time to obtain the first results and delay between two consecutive results) in the RAM-model of computation. This is opposite to top-k query processing trying to minimize the number of I/O accesses \cite{IlyasBS08,FingerP09}. The considered class of queries \cite{TziavelisAGRY-pvldb20} is, however, quite different from ours, since their full CQs do not include projections, counting quantifiers and threshold conditions. Although in recent unpublished work \cite{tziavelis2020TODS}, they also address CQs with projections, they mainly focus on ranked enumeration instead of considering unranked enumeration as in our case. 
%\angela{We can also go deeper and mention the difference between free-connex acyclicity in their case and bounded star-size and bounded free-connex tree-width here. We can also mention the fact that our algorithms are proactively exploiting the constant threshold while their algorithms do not.}
%\dominik{Agree. After refactoring, we have some space. So these few sentences can be useful.}


\paragraph{Sampling Answers}

Sampling query answers was identified as an important data management task by Chaudhuri at al. \cite{ChaudhuriMN99}, who proposed a simple algorithm for sampling the join $S \bowtie T$ by sampling a tuple $s \in S$ with weight $|T \ltimes \{s\}|$ and then uniformly sampling a tuple $t \in T \ltimes \{s\}$. Using the \emph{alias method} for weighted sampling \cite{Vose91,Walker77}, this algorithm can be implemented in such a way that after a linear preprocessing phase, independent samples can be obtained in constant time. 
% Excellent pedagogic explanation of the alias method by Keith Schwarz:
%https://www.keithschwarz.com/darts-dice-coins/
This approach can be  generalized to acyclic full CQs \cite{ZhaoC0HY18}, leveraging the linear algorithm for counting answers to acyclic full CQs (see \cite{Pichler_Skritek_2013}).
Our sampling algorithm generalizes this result  in three ways. (1) We handle non-acyclic CQs, allowing the complexity to grow with the tree-width of the query. It is routine to lift our approach to generalized hypertree-width, and thus recover the case of acyclic queries as a special case of generalized hypertree-width 1, with the same complexity. (2) We can allow projection, at the cost of replacing tree-width with its faster growing free-connex variant. This again lifts easily to generalized hypertree-width. (3) We handle threshold queries, rather than just conjunctive queries. Here, lifting to generalized hypertree-width is possible under an additional assumption; namely, that the lower threshold is at least 1. A different approach to non-acyclic full CQs was recently proposed by Chen and Yi \cite{Chen20}; it provides a uniform sampling algorithm with \emph{expected} running time 
%$O(\frac{n^{\rho+1}}{m})$ where $n$ is the size of the database instance, $\rho$ is the fractional hypertree-width of the query, and $m$ is the number of answers to the query;
proportional to the product of the database size and the ratio between the AGM bound \cite{AtseriasGM13} on the number of answers to the underlying full CQ and the actual number of answers of the input query;
this is incomparable to constant-time sampling after polynomial-time preprocessing, offered by our approach. Finally, Arenas et al. \cite{arenas2020approximate} show that, assuming  $\mathsf{FPT} \neq \mathsf{W}[1]$ and $\mathsf{BPP} = \P$, a structural class of CQs admits a fully polynomial-time \emph{almost uniform} sampler iff the queries in the class have bounded tree-width. Here, \emph{almost uniform} means that the algorithm approximates the uniform distribution up to a multiplicative error; this is a weaker notion than uniform sampling.

%\paragraph{Quantified Graph Pattern Queries} 
%Recently, the work in \cite{FanWX16} has introduced quantified graph patterns (QGP), an extension of  graph patterns with counting quantifiers on edges. Counting quantifiers \cite{Mostowski57} of the form $\exists^{\geq k}$ allow asserting the existence of at least $k$ elements with a given property. These are a generalization of normal quantifiers, as $\exists^{\geq 1} \equiv \exists$ and $\exists^{\geq n} \equiv \forall$ (for domains of size $n$), and have been extensively studied in finite model theory \cite{Ebbinghaus95,Otto97,Libkin04}, in the context of extending the expressive power of various logics.  In order to express quantified pattern matching, the authors of \cite{FanWX16} build on conventional subgraph isomorphism, to incorporate quantifier checking and process negated edges. Despite the expressivity of QGPs, these cannot account for counting in the context of k-hop reachability, i.e., the number of indirect descendents, nor can they account for counting tuples of variables, as in our case. Moreover, the approach relies on isomorphism matching, while ours is based on homomorphisms. 

\paragraph{Counting quantifiers}

The $\exists^{\geq k}$ and $\exists^{\leq k}$ quantifiers were introduced by Mostowski \cite{Mostowski57} and have been extensively studied in finite model theory \cite{Ebbinghaus95,Otto97,Libkin04}, in the context of extending the expressive power of various logics.
Recently, Fan et al. \cite{FanWX16} considered \emph{quantified graph patterns} (QGP), an extension of graph patterns that associates counting quantifiers to pattern edges and allows expressing nested counting properties like having at least 5 friends, each with at least 2 pets. In contrast to threshold queries, QGPs are unable to count $k$-hop neighbours for $k\geq 2$, nor can they count tuples of variables. Moreover, QGPs adopt isomorphism matching, while threshold queries are consistent with the standard semantics of database queries and are based on homomorphisms. 


\paragraph{Aggregate Queries}
In the context of factorized databases, Bakibayev et al. \cite{bakibayev2013Aggregation} observed that pushing aggregation down through joins can speed up evaluating queries. These results can be reinterpreted in the context of tree decompositions \cite{OlteanuZ15}, but they optimize different aggregates in isolation and do not investigate the interplay between counting and existential quantification.
AJAR (aggregations and joins over annotated relations) \cite{joglekar2016ajar} and FAQs (functional aggregate queries) \cite{KhamisNR16} are two very general sister formalisms capturing, among others, conjunctive queries enriched with multiple aggregate functions. Because different aggregate functions are never commutative, the evaluation algorithms for both these formalisms require decompositions consistent with the order of aggregating operations. For example, when applied to counting answers to CQs, this amounts to free-connex decompositions, as in our Proposition \ref{prop:counting-freeconnex}. 
In contrast, we remove the free-connex assumption by showing that counting up to a threshold and existential quantification can be reordered at the cost of keeping limited additional information (of pseudopolynomial size). 

%Khamis et al. \cite{khamis2020functional} formulate the problem in which some of the input factors are defined by a collection of additive inequalities between variables. It is a generalized way of viewing a common type of aggregation query called a Functional Aggregate Query (FAQ), which authors see parallels in multiple scenarios other than databases, e.g., matrix multiplication, and logic. In this paper the authors propose two algorithms, InsideOut and PANDA. For acyclic join queries, those algorithms effectively reduce to pushing aggregates below joins in the query plans. On the other hand, there are several works on worst-case optimal joins \cite{koutris2016worst,veldhuizen2014Triejoin}. That papers present how to avoid large intermediate results during execution of multi-way join queries.Joglekar et al. \cite{joglekar2016ajar} propose how to generalize the work on worst-case optimal multi-way joins \cite{koutris2016worst,veldhuizen2014Triejoin} to aggregate queries. 
% sum, count, avg, min, max
%In the context of factorized databases, Bakibayev et al. \cite{bakibayev2013Aggregation} show that factorization connected with partial aggregation can effectively reduce the number of operations needed for query evaluation. %Moreover, they discuss how factorizations of query results can support the enumeration of tuples in desired orders as efficiently as listing them from sorted results.

\paragraph{Top-$k$ and any-$k$}

The potential of predefined thresholds to speed up query processing was first noticed by Carey and Kossmann \cite{Carey1997}, who explored ways of propagating thresholds down query plans. This early study only considered applying the thresholds directly to subplans, which made joins a formidable obstacle. In contrast, we first group the answers to subqueries by variables determined based on the structure of the whole query, and then apply thresholds within groups; this way we can push thresholds down through multi-way joins, guided by a tree decomposition of the query. While most follow-up work concerns the case of ranked answers, which we discuss below, NeedleTail \cite{Kim2018,Kim2018tech} specifically focuses on providing any $k$ answers to queries without \texttt{ORDER BY} clauses, but it only handles queries over single tables and those with key-foreign key joins, which dominate in the OLAP scenarios.
In the ranked scenario the goal is to compute top $k$ answers according to a specified order. The celebrated Threshold Algorithm \cite{Fagin2003},  operates on a single vertically-partitioned table, with each partition being managed by a different external service that only knows the scores of base tuples in its own partition, and produces $k$ tuples with the highest score while minimizing the number of reads. There are several extensions to more general join problems, such as Rank-Join \cite{ilyas2004supporting}, J* \cite{natsev2001supporting}, a-FRPA \cite{finger2009robust}, and LARA-J* \cite{mamoulis2007efficient}. Rank-Join integrates the joining and ranking tasks in one efficient operator and performs sorted access to get tuples from each data source. The J* algorithm adopts a top-$k$ join query model where scores are assumed to be attached to join results rather than base tuples. The algorithm is based on the A* search algorithm but maintains a priority queue of partial and complete join combinations ordered on the upper bounds of their total scores. While a-FRPA and LARA-J* attempt to minimize how deep down the list they have to go in each presorted input table until they can guarantee that the correct results have been determined. These approaches obtain a bound on the score of possible join results containing "unseen" tuples and update this bound after accessing an input tuple. Overall, the challenge of top-$k$ processing is ordering the answers according to their scores. The absence of this challenge in the unranked case makes room for more general methods and stronger complexity guarantees. 

%
%
%\paragraph{\texttt{LIMIT} clause optimization and interactive data analytics} Optimizing  queries with \texttt{LIMIT} clauses is recognized as a promising approach to supporting progressive interactive data analytics \cite{BattleS21}. Nonetheless,  to our knowledge there has been little study of this. Indeed, existing database systems are not optimized for queries with a \texttt{LIMIT} clause, typically supporting \texttt{LIMIT} operations in an all-or-nothing manner. We summarize progress in the research literature on optimizing \texttt{LIMIT} clauses.  Kim et al.\ propose NEEDLETAIL, a data exploration engine providing two methods to efficiently retrieve any-$k$ valid records for arbitrary queries \cite{Kim2018,Kim2018tech}. The first algorithm, called DENSITY-OPTIMAL, optimizes for density and is based on the threshold algorithm introduced by Fagin et al.\ \cite{Fagin2003}. This method uses a DENSITYMAP index, a lightweight in-memory indexing structure to retrieve the densest blocks until $k$ valid records are found. The second algorithm, called LOCALITY-OPTIMAL, prioritizes locality rather than density. It identifies the shortest sequence of blocks that guarantee $k$ valid records. \dominik{Should we also cite Xu, Liqi PhD thesis?} Another proposal was presented by Carey and Kossmann \cite{Carey1997}. Here two policies are presented to exploit cardinality limits in relational query plans. The first policy, called \emph{conservative}, avoids restarts by restricting stop operator placement to safe locations in a query plan, e.g., leveraging key-foreign key relationships. 
%%In this approach, a stop operator is applied to a tuple stream if every tuple in that stream is guaranteed to generate at least one tuple of the overall query result. 
%The second policy, called \emph{aggressive}, allows placing stop operators at unsafe locations in a query plan. 
%Here an optimizer considers a stop insertion at each point in a query plan tree where the first column of the query with \texttt{ORDER BY} can be computed. 
%Our work differs from this, as we also support counting, enumeration, sampling, and do not require that query plans be modified with \texttt{STOP AFTER} operators. 
%
% \paragraph{Top-$k$ answers}
%Top-$k$ processing is a relatively active line of research. One of the important top-$k$ approaches is the Threshold Algorithm \cite{Fagin2003}, for which Fagin et al.\ received the 2014 Gödel Prize. This algorithm operates on a single table that is partitioned vertically, with each partition being managed by a different external service that knows the ranking only for its partition. In this approach, the scores are assumed to be attached to base tuples. A query is required to report the $k$ tuples with the highest scores. On the other hand, there are several extensions of the idea to more general join problems, such as Rank-Join \cite{ilyas2004supporting}, J* \cite{natsev2001supporting}, a-FRPA \cite{finger2009robust}, and LARA-J* \cite{mamoulis2007efficient}. Rank-Join integrates the joining and ranking tasks in one efficient operator and performs sorted access to get tuples from each data source. The J* algorithm adopts a top-$k$ join query model where scores are assumed to be attached to join results rather than base tuples. The algorithm is based on the A* search algorithm but maintains a priority queue of partial and complete join combinations ordered on the upper bounds of their total scores. While a-FRPA and LARA-J* attempt to minimize how deep down the list they have to go in each presorted input table until they can guarantee that the correct results have been determined. These approaches obtain a bound on the score of possible join results containing "unseen" tuples and update this bound after accessing an input tuple. Expressing a top-$k$ query requires the capability of ordering the tuples according to their scores, which is different from our approach.



%Papers we should mention:
%\begin{itemize}
%    \item \cite{TziavelisAGRY-pvldb20} is a very recent paper on full CQs.
%\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> tikzlibrarypie.code.tex <==
% SPDX-License-Identifier: GPL-2.0-only OR LPPL-1.3c
\RequirePackage{scalefnt}

%
% Utilities
%

\def\pgfpie@ifx#1#2{%
  \ifx#1#2%
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifdim#1#2#3{%
  \ifdim\dimexpr#1\relax#2\dimexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifnum#1#2#3{%
  \ifnum\numexpr#1\relax#2\numexpr#3\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@ifodd#1{%
  \ifodd\numexpr#1\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

\def\pgfpie@newif#1{%
  \csname newif\expandafter\endcsname\csname ifpgfpie@#1\endcsname
  \expandafter\def\csname pgfpie@if#1\expandafter\endcsname\expandafter{%
    \csname ifpgfpie@#1\endcsname
      \expandafter\pgfutil@firstoftwo
    \else
      \expandafter\pgfutil@secondoftwo
    \fi}%
}

%
% Constants for text comparison
%

\def\pgfpie@text@inside{inside}
\def\pgfpie@text@legend{legend}
\def\pgfpie@sum@c{100}
\def\pgfpie@sum@auto{auto}

% args:
% #1: begin angle
% #2: end angle
% #3: number
% #4: label
% #5: explode
% #6: fill color
% #7: radius
% #8: center
\def\pgfpie@slice#1#2#3#4#5#6#7#8{%
  \pgfmathparse{0.5*(#1)+0.5*(#2)}
  \let\pgfpie@midangle\pgfmathresult

  \path (#8) -- ++({\pgfpie@midangle}:{#5}) coordinate (pgfpie@O);

  \pgfmathparse{(#7)+(#5)}
  \let\pgfpie@radius\pgfmathresult
  
  % slice
  \draw[line join=round,fill={#6},\pgfpie@style] (pgfpie@O) -- ++({#1}:{#7}) arc ({#1}:{#2}:{#7}) -- cycle;

  \pgfmathparse{min(((#2)-(#1)-10)/110*(-0.3),0)}
  \pgfmathparse{(max(\pgfmathresult,-0.5) + 0.8)*(#7)}
  \let\pgfpie@innerpos\pgfmathresult

  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    % label and number together
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#4}\\\pgfpie@numbertext{#3}};
  }{%
    % label
    \pgfpie@ifhidelabel{}{%
      \pgfpie@iflegend{}{%
        \path (pgfpie@O) -- ++ ({\pgfpie@midangle}:{\pgfpie@radius})
        node[inner sep=0, \pgfpie@text={\pgfpie@midangle:#4}]{};
      }%
    }%

    % number
    \path (pgfpie@O) -- ++({\pgfpie@midangle}:{\pgfpie@innerpos}) node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\def\pgfpie@findColor#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@colorLength))}%
  \let\pgfpie@ci\pgfmathresult
  \foreach \pgfpie@c [count=\pgfpie@j from 0] in \pgfpie@color {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ci}{%
      \xdef\pgfpie@thecolor{\pgfpie@c}%
      \breakforeach
    }{}%
  }
}

\def\pgfpie@findExplode#1{%
  \pgfmathparse{int(mod(#1,\the\pgfpie@explodeLength))}%
  \let\pgfpie@ei\pgfmathresult
  \foreach \pgfpie@e [count=\pgfpie@j from 0] in \pgfpie@explode {%
    \pgfpie@ifnum{\pgfpie@j}{=}{\pgfpie@ei}{%
      \xdef\pgfpie@theexplode{\pgfpie@e}%
      \breakforeach
    }{}%
  }%
}

% #1: bottom left point
% #2: size
% #3: number
% #4: color
% #5: text
\def\pgfpie@square#1#2#3#4#5{%
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node[align=center]
    {\pgfpie@scalefont{#3}\pgfpie@labeltext{#5}\\\pgfpie@numbertext{#3}} ++(#2);
  }{%
    \draw[fill={#4},\pgfpie@style] (#1) rectangle node
    {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}} ++(#2);
  }%
}

% #1: pos
% #2: radius
% #3: number
% #4: color
% $5: style
% $6: label
\def\pgfpie@cloud#1#2#3#4#5#6{%
  \draw[fill=#4, #5] (#1) circle[radius=#2];
  \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{%
    \node[align=center] at (#1) {\pgfpie@scalefont{#3}\pgfpie@labeltext{#6}\\\pgfpie@numbertext{#3}};
  }{%
    \node at (#1) {\pgfpie@scalefont{#3}\pgfpie@numbertext{#3}};
  }%
}

\newdimen\pgfpie@angleEnd
\newcount\pgfpie@explodeLength
\newcount\pgfpie@colorLength
\newcount\pgfpie@sliceLength

\pgfqkeys{/pgfpie}{%
  explode/.store in=\pgfpie@explode,
  color/.store in=\pgfpie@color,
  radius/.store in=\pgfpie@radius,
  pos/.store in=\pgfpie@pos,
  style/.store in=\pgfpie@style,
  before number/.store in=\pgfpie@beforenumber,
  after number/.store in=\pgfpie@afternumber,
  text/.store in=\pgfpie@text,
  sum/.store in=\pgfpie@sum,
  rotate/.store in=\pgfpie@rotate,
}

\pgfpie@newif{polar}
\pgfqkeys{/pgfpie}{polar/.is if=pgfpie@polar}

\pgfpie@newif{legend}

\pgfpie@newif{square}
\pgfqkeys{/pgfpie}{square/.is if=pgfpie@square}

\pgfpie@newif{cloud}
\pgfqkeys{/pgfpie}{cloud/.is if=pgfpie@cloud}

\pgfpie@newif{scalefont}
\pgfqkeys{/pgfpie}{scale font/.is if=pgfpie@scalefont}
\def\pgfpie@scalefont#1{%
  \pgfpie@ifscalefont{%
    \pgfmathparse{(#1) / (\pgfpie@sum) * 3 + 0.9}%
    \scalefont{\pgfmathresult}%
  }{}%
}

\pgfpie@newif{hidenumber}
\pgfqkeys{/pgfpie}{hide number/.is if=pgfpie@hidenumber}
\def\pgfpie@numbertext#1{%
  \pgfpie@ifhidenumber{}{%
    \pgfpie@beforenumber#1\pgfpie@afternumber
  }%
}

\pgfpie@newif{hidelabel}
\pgfqkeys{/pgfpie}{hide label/.is if=pgfpie@hidelabel}
\def\pgfpie@labeltext#1{\pgfpie@ifhidelabel{}{#1}}

\tikzaddtikzonlycommandshortcutlet{\pie}{\pgfpie@pie}%

\def\pgfpie@pie{%
  \pgfutil@ifnextchar[{\pgfpie@@pie}{\pgfpie@@pie[]}%
}

\def\pgfpie@@pie[#1]#2{%
  % load default parameters
  \pgfqkeys{/pgfpie}{
    explode=0,
    color={blue!60, cyan!60, yellow!60, orange!60, red!60,
      blue!60!cyan!60, cyan!60!yellow!60, red!60!cyan!60,
      red!60!blue!60, orange!60!cyan!60},
    radius=3,
    pos={0,0},
    style={thick},
    before number=,
    after number=,
    text=label,
    sum=100,
    rotate=0,
    polar=false,
    square=false,
    cloud=false,
    scale font=false,
    hide number=false,
    hide label=false,
    every pie/.try,
  }%
  % load user's parameters
  \pgfqkeys{/pgfpie}{#1}%
  % add percentage automatically
  \pgfpie@ifx\pgfpie@sum\pgfpie@sum@c{%
    \pgfqkeys{/pgfpie}{after number=\%}%
    \pgfqkeys{/pgfpie}{#1}%
  }{}%

  % legend or not
  \pgfpie@ifx\pgfpie@text\pgfpie@text@legend{%
    \pgfpie@legendtrue
  }{%
    \pgfpie@legendfalse
  }%

  % handle sum
  \pgfpie@ifx\pgfpie@sum\pgfpie@sum@auto{%
    % sum all input
    \xdef\pgfpie@sum{0}%
    \foreach \pgfpie@p/\pgfpie@t in {#2} {%
      \pgfmathparse{(\pgfpie@sum) + (\pgfpie@p)}%
      \xdef\pgfpie@sum{\pgfmathresult}%
    }%
  }{}%

  % init counters
  \global\pgfpie@explodeLength=0
  \foreach \pgfpie@e in \pgfpie@explode {%
    \global\advance\pgfpie@explodeLength by 1
  }%

  \global\pgfpie@colorLength=0
  \foreach \pgfpie@c in \pgfpie@color {%
    \global\advance\pgfpie@colorLength by 1
  }%
  
  \pgfmathsetlength{\pgfpie@angleEnd}{0}%

  \global\pgfpie@sliceLength=0
  \foreach \pgfpie@p/\pgfpie@e in {#2} {%
    \global\advance\pgfpie@sliceLength by 1
  }%

  \pgfpie@ifsquare{%
    \pgfpie@pie@square{#2}%
    }{\pgfpie@ifcloud{\pgfpie@pie@cloud{#2}%
      }{\pgfpie@pie@circle{#2}}}

  % legend
  \pgfpie@ifhidelabel{}{%
    \pgfpie@iflegend{%
      \pgfpie@legend{#2}%
  }{}}%
}

\def\pgfpie@pie@square#1{%
  \pgfmathparse{(\pgfpie@radius)*2}
  \xdef\pgfpie@verticalLength{\pgfmathresult}
  \xdef\pgfpie@horizontalLength{\pgfmathresult}
  \path (\pgfpie@pos) -- ++({-\pgfpie@radius},{-\pgfpie@radius}) coordinate (pgfpie@start);
  \pgfmathparse{(\pgfpie@verticalLength) * (\pgfpie@horizontalLength) / (\pgfpie@sum)}
  \let\pgfpie@squareUnit\pgfmathresult

  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@ifdim{\pgfpie@verticalLength cm}{>}{\pgfpie@horizontalLength cm}{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@horizontalLength)}
      \let\pgfpie@height\pgfmathresult
      
      \pgfpie@square{pgfpie@start}{\pgfpie@horizontalLength,\pgfpie@height}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@horizontalLength},{\pgfpie@height*0.5})
            node[inner sep=0, \pgfpie@text={0:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{\pgfpie@verticalLength - \pgfpie@height}
      \xdef\pgfpie@verticalLength{\pgfmathresult}
      \path (pgfpie@start) -- ++(0, \pgfpie@height) coordinate (pgfpie@start);
    }{%
      \pgfmathparse{(\pgfpie@p) * (\pgfpie@squareUnit) / (\pgfpie@verticalLength)}%
      \let\pgfpie@width\pgfmathresult

      \pgfpie@square{pgfpie@start}{\pgfpie@width,\pgfpie@verticalLength}
      {\pgfpie@p}
      {\pgfpie@thecolor}
      {\pgfpie@t}
      %label
      \pgfpie@iflegend{}{%
        \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
          \pgfpie@ifhidelabel{}{%
            \path (pgfpie@start) -- ++({\pgfpie@width*0.5},{\pgfpie@verticalLength})
            node[inner sep=0, \pgfpie@text={90:{\pgfpie@t}}]{};
          }%
        }%
      }%

      \pgfmathparse{(\pgfpie@horizontalLength) - (\pgfpie@width)}%
      \xdef\pgfpie@horizontalLength{\pgfmathresult}%
      \path (pgfpie@start) -- ++({\pgfpie@width},0) coordinate (pgfpie@start);
    }%
  }%
}

\def\pgfpie@pie@cloud#1{%
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    % find explode
    \pgfpie@findExplode{\pgfpie@i}
    \def\pgfpie@cloudGap{(\pgfpie@theexplode) + 0.1}
    \pgfmathparse{sqrt((\pgfpie@p) / (\pgfpie@sum)) * (\pgfpie@radius)}
    \let\pgfpie@cloudR\pgfmathresult
    \pgfpie@ifnum{\pgfpie@i}{=}{0}{%
      % first cloud
      \coordinate (pgfpie@O) at (\pgfpie@pos);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{180+(\pgfpie@rotate)}
    }{\pgfpie@ifnum{\pgfpie@i}{=}{1}{%
      % second cloud
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
      \xdef\pgfpie@cloudExtendDir{45+(\pgfpie@rotate)}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}) coordinate (pgfpie@O);
    }{%
      % next cloud
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudRtwo)}
      \let\pgfpie@la\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRone)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lb\pgfmathresult
      \pgfmathparse{(\pgfpie@cloudRtwo)+(\pgfpie@cloudGap)+(\pgfpie@cloudR)}
      \let\pgfpie@lc\pgfmathresult
      \pgfmathparse{(\pgfpie@la)^2+(\pgfpie@lc)^2-(\pgfpie@lb)^2}
      \let\pgfpie@tmp\pgfmathresult
      \pgfmathparse{180 - acos((\pgfpie@tmp) / 2 / (\pgfpie@la) / (\pgfpie@lc))}
      \let\pgfpie@cloudRot\pgfmathresult
      \pgfpie@ifodd{\pgfpie@i}{%
        \pgfmathparse{-(\pgfpie@cloudRot)}
        \let\pgfpie@cloudRot\pgfmathresult
      }{}%
      \pgfmathparse{(\pgfpie@cloudExtendDir) - (\pgfpie@cloudRot)}
      \xdef\pgfpie@cloudExtendDir{\pgfmathresult}
      \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@lc}) coordinate (pgfpie@O);
      \xdef\pgfpie@cloudRone{\pgfpie@cloudRtwo}
      \xdef\pgfpie@cloudRtwo{\pgfpie@cloudR}
    }}%

    % find color
    \pgfpie@findColor{\pgfpie@i}

    \pgfpie@cloud{pgfpie@O}{\pgfpie@cloudR}{\pgfpie@p}
    {\pgfpie@thecolor}{\pgfpie@style}{\pgfpie@t}

    % label
    \pgfpie@iflegend{}{%
      \pgfpie@ifx\pgfpie@text\pgfpie@text@inside{}{%
        \pgfpie@ifhidelabel{}{%
          \path (pgfpie@O) -- ++({\pgfpie@cloudExtendDir}:{\pgfpie@cloudR})
          node[inner sep=0, \pgfpie@text={\pgfpie@cloudExtendDir:{\pgfpie@t}}] {};
        }%
      }%
    }%
  }%
}

\def\pgfpie@pie@circle#1{%
  \pgfpie@ifpolar{%
    \xdef\pgfpie@maxValue{0}
    \foreach \pgfpie@p/\pgfpie@e in {#1} {
      \pgfmathparse{\pgfpie@p}%
      \pgfpie@ifdim{\pgfpie@maxValue pt}{<}{\pgfmathresult pt}{%
        \xdef\pgfpie@maxValue{\pgfpie@p}
      }{}%
    }
    \pgfmathparse{(\pgfpie@sum) / \the\pgfpie@sliceLength}
    \xdef\pgfpie@polarangle{\pgfmathresult}
    \pgfmathparse{(\pgfpie@radius) / sqrt(\pgfpie@maxValue)}
    \xdef\pgfpie@polarRadiusUnit{\pgfmathresult}
  }{%
    \xdef\pgfpie@theradius{\pgfpie@radius}%
  }

  \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  % drawing loop
  \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
  {
    \pgfmathsetlength{\pgfpie@angleEnd}{\pgfpie@angleBegin}
    \pgfpie@ifpolar{%
      % Polar area diagram
      \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@polarangle}
      \pgfmathparse{sqrt(\pgfpie@p) * (\pgfpie@polarRadiusUnit)}
      \xdef\pgfpie@theradius{\pgfmathresult}
    }{%
    % normal pie
    \pgfmathaddtolength{\pgfpie@angleEnd}{\pgfpie@p}
    }

    % find explode
    \pgfpie@findExplode{\pgfpie@i}

    % find color
    \pgfpie@findColor{\pgfpie@i}
    \pgfpie@slice{(\pgfpie@angleBegin)/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\the\pgfpie@angleEnd/(\pgfpie@sum)*360+(\pgfpie@rotate)}
    {\pgfpie@p}
    {\pgfpie@t}
    {\pgfpie@theexplode}
    {\pgfpie@thecolor}
    {\pgfpie@theradius}
    {\pgfpie@pos}
    \xdef\pgfpie@angleBegin{\the\pgfpie@angleEnd}
  }
}

\def\pgfpie@legend#1{%
  \coordinate[xshift=0.8cm,
  yshift={(\the\pgfpie@sliceLength*0.5+1)*0.5cm}] (pgfpie@legendpos) at
  (current bounding box.east);

  \scope[node distance=0.5cm]
    \foreach \pgfpie@p/\pgfpie@t [count=\pgfpie@i from 0] in {#1}
    {
      \pgfpie@findColor{\pgfpie@i}
      \node[draw, fill={\pgfpie@thecolor}, \pgfpie@style, below of={pgfpie@legendpos}, label={0:{\pgfpie@t}}] (pgfpie@legendpos) {};
    }
  \endscope
}

